KYChain: User-Controlled KYC Data Sharing and Certification

Under Know Your Customer (KYC) regulations, financial institutions are required to verify the identity and assess the trustworthiness of any new client during on-boarding, and maintain up-to-date records for risk management. These processes are time consuming, expensive, typically have sub-par record-keeping steps, and disadvantage clients with nomad lifestyle. In this paper, we introduce KYChain as a privacy-preserving certification mechanism that allows users to share (certified) up-to-date KYC data across multiple financial institutions. We base KYChain on immutable ledgers and show that it offers confidentiality and certification compliance of KYC data.

==> application.tex <==


\section{Application: Know Your Customer}

The core of Know Your Customer is rigorous protocols for establishing the identify of potential clients/customers, measuring their degree of trustworthiness, and maintaining continues monitoring. 
%
%that you can expect from them, and  
%
%user identity by running a {\em Customer Identification Program}.

\paragraph{Parties}

\paragraph{Customer Identification Program}

Typical identification procedures consist of establishing the name, data of birth, address and personal identification number. This process is handled by our registration procedure. 

One strategy is to apply an enhancement of the verification mechanism that online mobile banks use, i.e., Monzo. Users fill in a series of forms that contain among other: their phone number, full name, current living address. This is coupled with a scan of their valid identity card or passport, and a recording that clearly shows their face. 

The verification consists of checking validity of documents-via communication with competent authorities, e.g. police, and verifying the person recorded matches the person on the scan document. Additional steps can be performed to validate the information in the recording w.r.t. their information on the form or scan document.

This type of registration mirrors the registration users typically face when opening in an account at any well established banks, and suffers from the same concern: people honestly registering, but then giving the account to others. Continued verification of the ownership for an account, with update of their personal information would mitigate this problem.  
		


\paragraph{Customer Due Diligence}

- use policy, and certificates from other banks

Clients do no present the same level of risk
Some clients/users have a higher risk of money laundering or terrorist funding

\paragraph{On Going Monitoring}

- certifiers are given access to documents, and can identify their transaction in the ledger

- any change/update for any document, via the ledger, would be detected. Banks would be able to request a new certification request, and run \ProofVerify with the user.

\paragraph{Digital Nomads}
- we can use offline registration, with a key-derivation algorithm over a password. 
- bank can handle the submit for the user, the user needs just the password, and valid id




%\subsection{Extensions and Limitations}
